A Numerical Method for a Nonlocal Form of Richards' Equation Based on Peridynamic Theory

Forecasting water content dynamics in heterogeneous porous media has significant interest in hydrological applications; in particular, the treatment of infiltration when in presence of cracks and fractures can be accomplished resorting to peridynamic theory, which allows a proper modeling of non localities in space. In this framework, we make use of Chebyshev transform on the diffusive component of the equation and then we integrate forward in time using an explicit method. We prove that the proposed spectral numerical scheme provides a solution converging to the unique solution in some appropriate Sobolev space. We finally exemplify on several different soils, also considering a sink term representing the root water uptake.

==> AMSLaTeXm.tex <==
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{ax}{Axiom}
\newtheorem{claim}[thm]{Claim}
\newtheorem{fact}[thm]{Fact}

\theoremstyle{definition}
%\newtheorem{defn}{Definition}[section]
%\newtheorem{rem}{Remark}[section] 
%\newtheorem{ass}{Assumption}[section] 
%\newtheorem{asss}{Assumptions}[section] 
%\newtheorem{exm}{Example}[section]
%\newtheorem{prob}{Problem}[section]

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{rems}[thm]{Remarks}
\newtheorem{ass}[thm]{Assumption} 
\newtheorem{asss}[thm]{Assumptions} 
\newtheorem{exm}[thm]{Example}
\newtheorem{prob}[thm]{Problem}
 
\theoremstyle{remark}

\numberwithin{equation}{section}

\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}

\font\eightrm=cmr8
\font\fiverm=cmr5
\newcommand{\stext}[1]{\text{\eightrm #1 }}
\newcommand{\sstext}[1]{\text{\fiverm #1 }}

\newcommand{\etalchar}[1]{$^{#1}$}

\def\bdots{{.^{\,\dps.^{\,\dps.}}}}
\def\svdots{\vbox{\baselineskip=1.5pt\lineskiplimit=0pt
	\kern1.5pt \hbox{$\ss .$}\hbox{$\ss .$}\hbox{$\ss .$}}}
\def\sdots{{\ss{\dots}}}
\def\sddots{\mathinner{\raise3pt\vbox{\hbox{$\ss .$}}
    \raise1.5pt\hbox{$\ss .$}\hbox{$\ss .$}}}
\def\towith#1{\ {\mathop{\to}\limits_{#1}}\ }
\def\ttowith#1{\ {\mathop{\longrightarrow}\limits_{#1}}\ }
\def\toappl#1{\ {\mathop{\to}\limits^{#1}}\ }
\def\ttoappl#1{\ {\mathop{\longrightarrow}\limits^{#1}}\ }
\def\otappl#1{\ {\mathop{\leftarrow}\limits^{#1}}\ }
\def\ottappl#1{\ {\mathop{\longleftarrow}\limits^{#1}}\ }

\newcommand{\B}{{\mathcal B}}
\newcommand{\E}{{\mathcal E}}
\newcommand{\M}{{\mathcal M}}
\newcommand{\X}{{\mathcal X}}
\newcommand{\Y}{{\mathcal Y}}
\newcommand{\K}{{\mathcal K}}
\newcommand{\U}{{\mathcal U}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\N}{{\mathbb N}}
\renewcommand{\P}{{\mathbb P}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\Rn}{{\R^n}}
\newcommand{\Cn}{{\C^n}}
\newcommand{\Rnxn}{{\R^{n\times n}}}
\newcommand{\Cnxn}{{\C^{n\times n}}}
\newcommand{\Rmxn}{{\R^{m\times n}}}
\newcommand{\Cmxn}{{\C^{m\times n}}}
\newcommand{\Rmxm}{{\R^{m\times m}}}
\newcommand{\Cmxm}{{\C^{m\times m}}}
\newcommand{\Fmxn}{{\F^{m\times n}}}
\newcommand{\Fnxn}{{\F^{n\times n}}}

\newcommand{\cont}{{\mathcal C}} 
\newcommand{\pol}{{\mathcal P}}

\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\re}{\operatorname{Re}}
\newcommand{\im}{\operatorname{Im}}
\newcommand{\per}{\operatorname{per}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\trace}{\operatorname{trace}}
\newcommand{\grad}{\operatorname{grad}}
\newcommand{\cond}{\operatorname{cond}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\spect}{\operatorname{Sp}}
\newcommand{\range}{\operatorname{range}}
\newcommand{\ncl}{{\operatorname{cl}_{\operatorname{num}} }}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\lcm}{\operatorname{lcm}}
\newcommand{\eps}{\varepsilon}
\newcommand{\half}{{\frac{1}{2}}}
\newcommand{\thalf}{\tfrac{1}{2}}
\newcommand{\itext}[1]{{\qquad\text{#1}\qquad}}
\newcommand{\abs}[1]{\left| #1 \right|}
\newcommand{\tabs}[1]{| #1 |}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}

\newcommand{\tnorm}[1]{\Vert #1 \Vert}
\newcommand{\vnorm}[1]{\vert #1 \vert}
\newcommand{\Vnorm}[1]{\left\vert #1 \right\vert}
\newcommand{\mnorm}[1]{\vert #1 \vert}
\newcommand{\Mnorm}[1]{\left\vert #1 \right\vert}
\newcommand{\norm}[1]{\left\Vert #1 \right\Vert}
\newcommand{\supnorm}[1]{\Vert #1 \Vert_\infty}
\newcommand{\inprod}[1]{\left\langle #1 \right\rangle}
\newcommand{\wnorm}[1]{\vnorm{ #1 }_{\sss\mat{W}}}
\newcommand{\winprod}[1]{\inprod{ #1}_{\sss\mat{W}}}

\newcommand{\ontop}[2]{\genfrac{}{}{0pt}{}{#1}{#2}}
\newcommand{\trestr}[2]{ {#1}_{\vert_{#2}}}%old definition
%\newcommand{\trestr}[2]{ {#1}{\big|_{#2}}}
\newcommand{\restr}[2]{ {#1}_{\big|_{\textstyle{{#2}}}}}%old definition
%newcommand{\restr}[2]{ {#1}{\bigg|_{\textstyle{{#2}}}}}
\newcommand{\srestr}[2]{ {#1}{|_{\scriptstyle{{#2}}}}}
\newcommand{\subst}[2]{ {\big/_{#1}^{#2}}}
\newcommand{\set}[2]{ \left\{ {#1}\,\big\vert\, {#2}\right\}}
\newcommand{\inbr}[1]{ \left\{ \,{#1}\,\right\}}
\newcommand{\seq}[2]{ \left\{ {#1}\right\}_{#2}}
\newcommand{\binomial}[2]{ \left( \ontop{#1}{#2}\right)}
\newcommand{\sbinomial}[2]{ {\textstyle\left( \ontop{#1}{#2}\right)}}
\newcommand{\arr}[1]{ \begin{matrix} #1 \end{matrix}}
\newcommand{\sarr}[1]{ \begin{smallmatrix} #1 \end{smallmatrix}}
\newcommand{\smat}[1]{ \left[\begin{smallmatrix} #1 \end{smallmatrix}\right]}
\newcommand{\determinant}[1]{ \left\vert\begin{matrix} 
		#1 \end{matrix}\right\vert}
\newcommand{\bmat}[1]{ \begin{bmatrix}#1\end{bmatrix}}
\let\tilde\widetilde
\let\hat\widehat
\let\cc\c

\newcommand{\hf}{\null\hfill\null}
\newcommand{\dps}{\displaystyle}
\newcommand{\txs}{\textstyle}
\renewcommand{\ss}{\scriptstyle}
\newcommand{\sss}{\scriptscriptstyle}
\newcommand{\SDisplay}[1]{\newline$\dps\null\qquad #1$\newline}
\newcommand{\sDisplay}[1]{\newline$\dps\null\qquad #1$}

\newcommand{\eqalign}[1]{ \begin{aligned}#1\end{aligned}}

\newcommand{\trans}{\cap^{\:\!\!\!\!\! \vert \,\,\,\,}\!}
\newcommand{\transx}[1]{\ontop{\bigcap^{\:\!\!\!\!\! \vert \,\,\,\,}\!}{#1}}


\def\BGamma{{\boldsymbol{\Gamma}}} 
\def\BLambda{{\boldsymbol{\Lambda}}}
\def\BPhi{{\boldsymbol{\Phi}}} 
\def\BPsi{{\boldsymbol{\Psi}}} 
\def\balpha{{\boldsymbol{\alpha}}}
\def\bbeta{{\boldsymbol{\beta}}}
\def\bgamma{{\boldsymbol{\gamma}}}
\def\bdelta{{\boldsymbol{\delta}}}
\def\blambda{{\boldsymbol{\lambda}}}
\def\bnu{{\boldsymbol{\nu}}}
\def\bphi{{\boldsymbol{\phi}}}
\def\bpsi{{\boldsymbol{\psi}}}
\def\bsigma{{\boldsymbol{\sigma}}}
\renewcommand{\vec}[1]{{\boldsymbol{#1}}}
\newcommand{\mat}[1]{{\boldsymbol{#1}}}
\def\b{\vec{b}} 
\def\e{\vec{e}} 
\def\f{\vec{f}}
\def\g{\vec{g}} 
\def\h{\vec{h}} 
\def\l{\vec{l}}
\def\p{\vec{p}} 
\def\q{\vec{q}} 
\def\r{\vec{r}}
\def\s{\vec{s}}
\def\u{\vec{u}} 
\def\v{\vec{v}}
\def\w{\vec{w}} 
\def\x{\vec{x}}
\def\y{\vec{y}} 
\def\z{\vec{z}}
\def\bF{\vec {F}} 
\def\bP{\vec {P}} 
\def\bQ{\vec {Q}}
\def\A{\mat{A}} 
\def\BB{\mat{B}} 
\def\BC{\mat{C}} 
\def\BD{\mat{D}} 
\def\BE{\mat {E}} 
\def\BF{\mat {F}} 
\def\G{\mat{G}} 
\def\BI{\mat{I}} 
\def\BJ{\mat {J}}
\def\BP{\mat {P}} 
\def\BQ{\mat {Q}} 
\def\BR{\mat {R}}
\def\BS{\mat {S}} 
\def\BU{\mat {U}} 
\def\BY{\mat{Y}}
\newcommand{\nz}{\times}
\newcommand{\mc}{\text{\eightrm EPS}}
\newcommand{\var}[1]{{\eightrm #1}}
\def\vx{\vphantom{$\sum_j^j$}}

\def\yes{Yes}
\newcommand{\ForUsOnly}[1]{\ifx\UsOnly\yes {\em #1}\fi}

